On Groebner Basis in Monoid and Group Rings

Developed by Buchberger for commutative polynomial rings, Groebner Bases are frequently applied to solve algorithmic problems, such as the congruence problem for ideals. Until now, these ideas have been transmitted to different in part non-commutative and non-Noetherian algebras. Most of these approaches require an admissible ordering on terms. In this Ph.D.thesis, the concept of Groebner bases is generalized to finitely generated monoid and group rings. Reduction methods are applied to represent monoid and group elements and to describe the right-ideal congruence in the corresponding monoid and group rings, respectively. In general, monoids and especially groups do not offer admissible orderings anymore. Thus, the definition of an appropriate reduction relation is confronted with the following problems: On the one hand, it is difficult to guarantee termination. On the other hand, reduction steps are not compatible with multiplication anymore, so that the reduction relation does not necessarily generate a right-ideal congruence. In this thesis, several possibilities of defining reduction relations are presented and evaluated w.r.t. the described problems. The concept of saturation (i.e. the extension of a set of polynomials in such a way that the right-ideal congruence it generates can be captured by reduction) is applied to characterize Groebner bases relatively to the different reductions by s-polynomials. Using these concepts and special structural properties, it was possible to define special reduction relations for special classes of monoids (e.g., finite, commutative, or free) and for different classes of groups (e.g., finite, free, plain, context-free, or nilpotent) and to develop terminating algorithms for computing Groebner bases w.r.t. these reduction relations.

==> oddbits.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Miscellaneous Notes on Gr\"obner Bases}%\Rand{}{~}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{On Gr\"obner Bases in Finitely Generated Commutative
         Monoid Rings}
In this section we will sketch how Buchberger's Algorithm can
 be lifted to quotient rings. 
The ideas are mainly the same as stated in \cite{De90}.
Let us start by recalling Buchberger's definition of reduction for a
 polynomial ring $\myk[X_1, \ldots , X_n]$.
%
\begin{definition}~\\
{\rm 
Let $p = \sum_{i = 1}^{n} c_{i} \skm t_{i}, g = \sum_{j = 1}^{m} d_{j} \skm s_{j}
 \in \myk[X_1, \ldots , X_n]$. \\
We say $g$ {\em  reduces} $p$ to $q$ at $c_k \skm t_k$ in one step,
 i.e., $p \red{}{\myr}{}{g} q$, if
\begin{enumerate}
\item[(a)] $s_1 \mm u = t_{k}$ for some $u \in {\cal T}$, and
\item[(b)] $q = p - c_k \skm d_1^{-1} \skm g \mrm u$.
\end{enumerate}
We write $p \red{}{\myr}{}{g}$ if there is a polynomial $q$ as defined above. \\
We can define $\red{*}{\myr}{}{}, \red{+}{\myr}{}{}$, and
 $\red{n}{\myr}{}{}$ as usual.
Reduction by a set $F \subseteq \myk[X_1, \ldots , X_n]$ is denoted by
 $p \red{}{\myr}{}{F} q$ and stands for  $p \red{}{\myr}{}{g} q$ for some $g \in F$,
 also written as  $p \red{}{\myr}{}{g \in F} q$.
}
\end{definition} 
%
As we are interested in finitely generated commutative monoids only,
 let us assume that our monoid $\m$ is presented by a set of generators
 $\Sigma = \{ X_1, \ldots , X_n \}$ and a set of relations
 $R = \{ (l_i,r_i) | 1 \leq i \leq k, l_i , r_i \in
 \free_c \}$\footnote{As
 before let $\free_c$ be the free commutative monoid generated by
 $\Sigma$.}.
Then we can view the set $R$ as a set of polynomials 
 $P_R = \{ l_i - r_i | (l_i,r_i) \in R \}$.
Let $P_T$ be the Gr\"obner basis of $P_R$.
Then $P_T$ is again a finite set consisting of polynomials of
 the form $l - r$, where $l,r \in \free_c$.
We can show that the monoid ring $\myk[\m]$ is in fact isomorphic to a quotient
 of the ordinary polynomial ring $\myk[X_1, \ldots , X_n]$.
%
\begin{lemma}~\\
{\sl
Let $\m$ be a commutative monoid generated by
 $\Sigma = \{ X_1, \ldots , X_n \}$ and the relations
 $R = \{ (l_i,r_i) | 1 \leq i \leq k \}$.
Further let $P_T$ be a Gr\"obner basis of $P_R$
 as described above.
Then $\myk[\m]$ is isomorphic to
 $\myk[X_1, \ldots , X_n]/ideal(P_{T})$.
}
\end{lemma}
\Ba{}~\\
 Loosely spoken, if $\m$ has a presentation $(\Sigma , R)$,
  then $\m$ can be viewed as a subset of the free monoid
  $\free_c$ generated by $\Sigma$.
 For two words $u,v \in \free_c$ we have $u =_{\m} v$ iff
  $u \id t_0 =_R t_1 =_R \ldots =_R t_n \id v$, where
  $t_i =_R t_{i+1}$ iff $(t_i = l \mm_{\free_c} s \mbox{ and } 
                          t_{i+1} = r \mm_{\free_c} s)$ or
                        $(t_{i+1}= l \mm_{\free_c} s \mbox{ and } 
                          t_{i} = r \mm_{\free_c} s)$
  for some $(l,r) \in R$ and $s \in \free_c$.
 The elements of $\m$ then correspond to the equivalence classes 
  $[w]_R$ for $w \in \free_c$, $[\lambda]_R$ represents the
  unit and multiplication can be defined as 
  $[u]_R \mm_{\m} [v]_R = [u \mm_{\free_c} v]_R$.
 Now if $P_T$ is a Gr\"obner basis correspomding to $P_R$,
  we know $\red{*}{\lr}{}{P_T} = \red{*}{\lr}{}{P_R}$.
 Further we can show $u =_R v$ iff $u \red{*}{\lr}{}{P_R} v$.
 Hence, we can use the reduction $\red{}{\myr}{}{P_T}$ in
  $\myk[X_1, \ldots, X_n]$ to compute unique representations for
  the elements of $\m$ giving us a one-to-one correspondence by
  defining the representant of $[w]_R$ to be the normalform of $w$
  with respect to $P_T$ in $\myk[X_1, \ldots, X_n]$, i.e., $w\nf{P_T}$.
\\
\qed
%
Now let us state how computation in our quotient structure is done.
By writing $p \in \myk[X_1, \ldots , X_n]/ideal(P_{T})$ we will
 always assume $p$ to be in normal form with respect to $P_T$.
%
\begin{definition}~\\
{\rm 
Let $p,q \in \myk[X_1, \ldots , X_n]/ideal(P_{T})$.
Then we can define addition and multiplication as follows:
\begin{enumerate}
\item $p +' q := (p + q)\nf{P_T}$
\item $p \mrm ' q := (p \mrm q)\nf{P_T}$
\end{enumerate}
where $+$ and $\mrm$ are the corresponding ring operations in
 $\myk[X_1, \ldots, X_n]$.
}
\end{definition}
%
Then $\myk[X_1, \ldots , X_n]/ideal(P_{T})$ together with $+'$ and 
 $\mrm '$ is a commutative ring with unit.
We will now introduce reduction to this structure.
%
\begin{definition}~\\
{\rm
Let $p,q,g \in \myk[X_1, \ldots , X_n]/ideal(P_{T})$ and
 $\red{}{\myr}{}{}$ Buchberger's reduction as defined in
 \ref{def.}.
Then we set
$p \red{}{\myr}{}{g} q$ if there exists a polynomial
 $q' \in \myk[X_1, \ldots, X_n]$ such that
 $p \red{}{\myr}{}{g} q'$ and $q = q'\nf{P_T}$.
\\
We can define $\red{*}{\myr}{}{}, \red{+}{\myr}{}{}$, and
 $\red{n}{\myr}{}{}$ as usual.
Reduction by a set $F \subseteq \myk[X_1, \ldots , X_n]/ideal(P_{T})$ is denoted by
 $p \red{}{\myr}{}{F} q$ and stands for  $p \red{}{\myr}{}{g} q$ for some $g \in F$,
 also written as  $p \red{}{\myr}{}{g \in F} q$.
}
\end{definition}
%
Then for this reduction we can state:
\begin{lemma}~\\
{\sl
Let $F \subseteq \myk[X_1, \ldots , X_n]/ideal(P_{T})$ and
 $p,q \in \myk[X_1, \ldots , X_n]/ideal(P_{T})$.
\begin{enumerate}
\item $\red{}{\myr}{}{F} \subseteq \red{*}{\myr}{}{F \cup P_T}$.
\item $p \red{}{\myr}{}{F} q$ implies $p > q$.
\item $\red{}{\myr}{}{F}$ is Noetherian.
\end{enumerate}
}
\end{lemma}
%
But although $\myk[X_1, \ldots , X_n]/ideal(P_{T})$ still is a Noetherian ring,
 many other properties of reduction are lost.
%
\begin{lemma}~\\
{\sl
Let $p,q,h \in \myk[X_1, \ldots , X_n]/ideal(P_{T})$, $h \neq 0$.
\begin{enumerate}
\item $p < q$ no longer implies $p \mrm ' h < q \mrm ' h$.
\item $p \red{}{\myr}{}{q}$ no longer implies $p \mrm ' h
  \red{}{\myr}{}{q}$.
\item $p \red{}{\myr}{}{p} 0$ no longer implies $p \mrm ' h
  \red{}{\myr}{}{p} 0$.
\item $\{ p \}$ need not be a Gr\"obner basis.
\end{enumerate}
}
\end{lemma}
%
We now can give a definition for Gr\"obner bases.
%
\begin{definition}~\\
{\rm
A set $G \subseteq \myk[X_1,\ldots,X_n]$ is said to be a {\em
 Gr\"obner basis}\/ of an ideal generated by a set 
 $F  \subseteq \myk[X_1,\ldots,X_n]$, if
\begin{enumerate}
\item $ideal(G) = ideal(F)$
\item $\red{*}{\myr}{}{G}$ is confluent.
\end{enumerate}
}
\end{definition}
%
The following lemma describes a way to compute such bases.
%
\begin{lemma}~\\
{\sl
Let $P_T$ be a Gr\"obner basis,
 $F \subseteq \myk[X_1, \ldots , X_n]/ideal(P_{T})$
 and let $\red{}{\myr}{}{F \cup P_T}$ be confluent on $\myk[X_1, \ldots,
 X_n]$.
Then $\red{}{\myr}{}{F}$ is also confluent.
}
\end{lemma}
%
The converse is not true.
But we can compute a (even reduced) Gr\"obner basis as follows:

Compute the reduced Gr\"obner basis $G'$ of $F \cup P_T$ in
 $\myk[X_1, \ldots, X_n]$ with respect to Buchberger's
 reduction without changing the polynomials in $P_T$.
Then the set $G := G' \backslash P_T$ is the reduced gr\"obner basis
 of $F$ in $\myk[X_1, \ldots, X_n]/ideal(P_T)$.
Computing the Gr\"obner basis of $F \cup P_T$ three kinds of
 s-polynomials can arise:
\begin{enumerate}
\item $f,g \in P_T$:
\\
      Then the corresponding s-polynomial can be omitted, as
       $P_T$ is already a Gr\"obner basis.
\item $f,g \in F$:
\\
      Then the s-polynomial corresponds to the commutative
       s-polynomial as defined in section \ref{section.}.
\item $f \in F$, $g \in P_T$:
\\
      Then the s-polynomial coressponds to the process of
       saturating $f$, in particular to the step of overlapping
       the head term of $f$ with the rule $(l,r)$ where $g = l-r$.
\end{enumerate}
We end up with a characterization of Gr\"obner bases as follows:
%
\begin{theorem}~\\
{\sl 
Let $G \subseteq \myk[X_1, \ldots, X_n]/ideal(P_T)$.
$G$ is a Gr\"obner basis if
\begin{enumerate}
\item for all $f,g \in G$, $spol(f,g) \red{*}{\myr}{}{G} 0$ and
\item for all $f \in G$, $g \in P_T$, $spol(f,g) \red{*}{\myr}{}{G} 0$.
\end{enumerate}
}
\end{theorem}
%
In fact the two reductions $\red{}{\myr}{}{}$ and $\red{}{\myr}{c}{}$ are
closely related and one can show the equivalence of the above
characterization to the following
\begin{theorem}~\\
{\sl 
Let $G \subseteq \myk[\m]$.
$G$ is a Gr\"obner basis if
\begin{enumerate}
\item for all $f,g \in G$, $spol(f,g) \red{*}{\myr}{c}{G} 0$ and
\item for all $f \in G$, every right multiple of $f$ has a
      commutative standard representation with respect to $G$.
\end{enumerate}
}
\end{theorem}

!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
TODO:
Beispiel fuer den Unterschied zwischen $\red{}{\myr}{r}{}$ und
 $\red{}{\myr}{}{}$.

Vergleiche GB bzgl. $\red{}{\myr}{r}{}$,GB bzgl. $\red{}{\myr}{c}{}$,
 GB bzgl. $\red{}{\myr}{}{}$ 
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{On Gr\"obner Bases in Finitely Generated Arbitrary
         Monoid Rings}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we show how a finitely generated  arbitary monoid
 ring can be viewed as a quotient of a free monoid ring and what
 consequences arise trying to lift reduction as defined e.g. by Mora
 to this structure.
 
We start by giving Mora's definition of reduction in free monoid
 rings as stated in \cite{Mo85}.
Let $\free$ denote a free monoid generated by a finite set $\Sigma$.
%
\begin{definition}\label{def.red.mora}~\\
{\rm
Let $\succ$ be a total admissible well-founded ordering on $\free$
 used to order the terms in the polynomials in $\myk[\free]$.
Let $p = \sum_{i = 1}^{n} a_{i} \skm w_{i}$,
 $g = \sum_{j = 1}^{m} b_{j} \skm v_{j} \in \myk[\free]$. \\
We say $g$ {\em reduces} $p$ to $q$ at $a_k \skm w_k$ in one step,
 i.e., $p \red{}{\myr}{}{g} q$, if
\begin{enumerate}
\item[(a)] $xv_1y = w_{k}$ for some $x,y \in \free$, where $v_1
  \succ v_j$, $2 \leq j \leq n$.
\item[(b)] $q = p - (a_k \skm b_1^{-1}) \skm x \mrm g \mrm y$.
\end{enumerate}
We write $p \red{}{\myr}{}{g}$ if there is a polynomial $q$ as defined above. \\
We can define $\red{*}{\myr}{}{}, \red{+}{\myr}{}{}$,
 $\red{n}{\myr}{}{}$ and  reduction by a set $F \subseteq \myk[\free]$ as usual, and
 $\red{*}{\lr}{}{F} = \,\,\,\equiv_{ideal(F)}$.
}
\end{definition}
%
As in the previous section we can assume that our monoid
 $\m$ is presented by its generators
 $\Sigma = \{ X_1, \ldots , X_n \}$ and relations
 $R = \{ (l_i,r_i) | 1 \leq i \leq k, l_i , r_i \in
 \free \}$.
Then we can view the set $R$ as a set of polynomials 
 $P_R = \{ l_i - r_i | (l_i,r_i) \in R \}$.
Unfortunately, in $\myk[\free]$ finite Gr\"obner bases no longer
 need to exist.
This problem is closely related to the fact that the word problem
 for arbitrary finitely presented monoids is undecidable.
%
\begin{theorem}\label{theo.wp}~\\
{\sl
Let $(\Sigma, T)$ be a finite Thue system with
 $T= \{ (l_i,r_i) | i = 1, \ldots , n \}$.
We can associate a system of polynomials with $T$ by setting
 $P_T= \{ l_i-r_i | i = 1, \ldots, n \} \subseteq
 {\myk[\Sigma^*]}$\footnote{$\myk[\free]$
 denotes the free monoid ring generated by $\Sigma$.}.
\\
Further let $u,v \in \free$.
Equivalent are:
\begin{enumerate}
\item $u \red{*}{\lr}{}{T} v$
\item $u-v \in ideal(P_T)$.
\end{enumerate}
}
\end{theorem}
\Ba{}~\\
$1 \R 2:$ \\
 Using induction on $k$ we show that $u \red{k}{\lr}{}{T} v$ implies
        $u - v \in ideal(P_T)$.\\
 In the base case $k = 0$ there is nothing to show, since
  $u-u =0 \in ideal(P_T)$.\\
 Let us assume that  $\tilde{u} \red{k}{\lr}{}{T} \tilde{v}$
  implies $ \tilde{u}-\tilde{v} \in ideal(P_T)$.\\
 Looking at $ u \red{k}{\lr}{}{T} u_{k}  \red{}{\lr}{}{T} v$ we find
 $u_{k}  \red{}{\lr}{}{T} v$ with $(l_j,r_j) \in T$.
\\
 Without loss of generality we can assume $u_k = xl_jy$ for
  some $x,y \in \Sigma^*$  
 giving us $v = xr_jy$, and written in terms of polynomials
 $v = u_k - x\mrm (l_j-r_j) \mrm y$\footnote{Recall that
 multiplication in the free monoid $\free$ is
 just concatenation.}.
 As $u-v = u- u_k + x \mrm (l_j-r_j) \mrm y$ and $u-u_k \in
 ideal(P_T)$ by our induction hypothesis,
 we get $u-v \in ideal(P_T)$.
\\
\\
$2 \R 1:$ \\
 We have to show that $u-v \in ideal(P_T)$ implies $u \red{*}{\lr}{}{T} v$.\\
 We know $u-v= \sum_{j=1}^{n} d_j \skm x_j \mrm (l_{i_j} - r_{i_j})
 \mrm y_j$, where
  $d_j \in \myk, x_j,y_j \in \free$.
 Therefore, by  showing the following stronger result we are done:
 A representation
 $ u - v = \sum_{j=1}^m p_j$ where $p_j = c_j \skm (w_j -w'_j)$,
 $c_j \in \myk$ and $w_j \red{+}{\lr}{}{T} w'_j$ implies 
 $u \red{*}{\lr}{}{T} v$.
\\
 Let $u - v = \sum_{j=1}^m p_j$ be such a representation.
 Further let $\succ$ be  an arbitrary total well-founded ordering
 on $\free$.
\\
 Depending on the  representation $\sum_{j=1}^m p_j$  and the ordering $\succ$ we define
  $t = max \{w_j,w'_j   \mid j = 1, \ldots m  \}$  and
  $K =$ number of $p_j$ containing $t$ as a term.
\\
 We will show our claim by induction on $(m,K)$, where 
  $(m',K') < (m,K)$ if and only if $m'<m$ or $(m'=m$ and $K'<K)$.
\\
 In case $m=0$, $u-v=0$ implies $u=v$ and hence $u \red{0}{\lr}{}{T} v$.
\\
 Now let $m>0$.
\\
 In case $K=1$, let $p_k$ be the polynomial containing
  $t$\footnote{We either have $p_k=c_k \skm (t-w'_k)$
  or $p_k=c_k \skm (w_k - t)$, where $c_k \in \{ 1, -1 \}$.}.
 Without loss of generality we can assume $u=t$ and $p_k=t-w'_k$.
 Using $p_k$ we can decrease $m$ by subtracting $p_k$ from $u-v$ giving us
  $w'_k-v = \sum_{j=1,j \neq k}^{m} p_j$.
 Since $u=t \red{*}{\lr}{}{T} w'_k$ and our induction
  hypothesis yields $w'_k \red{*}{\lr}{}{T} v$
  we get $u \red{*}{\lr}{}{T} v$.
\\
 In case $K>1$ there are two polynomials $p_k,p_l$ in
  the corresponding representation and without loss
  of generality we can assume $p_k = c_k \skm( t - w'_k)$ and $p_l =
 c_l \skm (t -w'_l)$\footnote{The case where $p_k = c_k \skm( w'_k - t)$ and $p_l =
 c_l \skm (w'_l - t)$ occur can be treated similar by modifying the coefficient.}.
\\
 If $w'_k = w'_l$  we can immediately decrease $m$ 
  by substituting the occurrence of $p_k+p_l$  by $(c_k + c_l) \skm p_l$.
\\
 Otherwise we can proceed as follows:
  \begin{eqnarray*}
  p_k + p_l & = & p_k \underbrace{-  c_k \skm c_l^{-1} \skm p_l + c_k  \skm c_l^{-1} \skm p_l}_{=0} + p_l \\
            & = & \underbrace{(-c_k \skm w'_k + c_k  \skm w'_l)}_{p'k} + (c_k \skm c_l^{-1} +1) \skm p_l \\
  \end{eqnarray*}
  where $p'_k = c_k \skm (w'_l - w'_k)$, $w'_k \red{*}{\lr}{}{T} t \red{*}{\lr}{}{T} w'_l$
  and $w'_l \neq w'_k$.
 In case $c_k \skm c_l^{-1} + 1=0$, i.e. $c_k=-c_l$, $m$ is decreased.
 On the other hand $p'_k$ does not contain $t$, i.e., if $m$ is not
 decreased $K$ is.
\\
\qed
%
This is nothing new as the congruence problem for two-sided ideals
 in free monoid rings is undecidable (compare \cite{KaWe90}).
Perhaps less obvious than this observation is the fact that
 the word problem for groups similarly reduces to the
 congruence problem for ideals in the
 free group ring.
%
\begin{theorem}~\\
{\sl
Let $(\Sigma, T \cup T_{I})$ be a finite group system with
 $T= \{ (l_i,r_i) | i = 1, \ldots , n \}$
 and $T_{I}= \{(\imath(a)a, \lambda),(a\imath(a), \lambda) | a \in\Sigma \}$.
We can associate a system of polynomials with $T$ by setting
 $P_T= \{ l_i-r_i | i = 1, \ldots, n \} \subseteq
 {\myk[\free_{fg}]}$\footnote{Without loss of generality we assume
 that $l_i$ and $r_i$ are in normal form with respect to $T_I$.}.
\\
Further let $u,v \in \Sigma^*$.
Equivalent are:
\begin{enumerate}
\item $u \red{*}{\lr}{}{T \cup T_{I}} v$
\item $u\nf{T_{I}}  -v\nf{T_{I}} \in ideal(P_T)$.
\end{enumerate}
}
\end{theorem}
\Ba{}~\\
$1 \R 2:$ \\
 Using induction on $k$ we show that $u \red{k}{\lr}{}{T \cup T_{I}} v$ implies
        $u\nf{T_{I}} - v\nf{T_{I}} \in ideal(P_T)$.\\
 In the base case $k = 0$ we have $u=v$ and, therefore,
  $u\nf{T_{I}}-u\nf{T_{I}} =0 \in ideal(P_T)$.\\
 Let us assume that  $\tilde{u} \red{k}{\lr}{}{T \cup T_{I}} \tilde{v}$ 
  implies $ \tilde{u}\nf{T_{I}}-\tilde{v}\nf{T_{I}} \in ideal(P_T)$.\\
 Looking at $ u \red{k}{\lr}{}{T \cup T_{I}} u_{k} 
 \red{}{\lr}{}{T \cup T_{I}} v$ we can distinguish:
      \begin{enumerate}
      \item $u_{k}  \red{}{\lr}{}{T} v$ with $(l,r) \in T$.
\\
            Without loss of generality we can assume $u_k = xly$ and
            $v = xry$ for some $x,y \in \Sigma^*$.
            Now $$u\nf{T_{I}}-v\nf{T_{I}} = u\nf{T_{I}}-
            \underbrace{u_k\nf{T_{I}} + xly\nf{T_{I}}}_{=0} -
            xry\nf{T_{I}}$$ and $xly\nf{T_{I}} - xry\nf{T_{I}} = x
            \mrm (l-r) \mrm y$.
            By our induction hypothesis  $u\nf{T_{I}}-u_k\nf{T_{I}}
            \in ideal(P_T)$ and, hence,  we get
            $u\nf{T_{I}}-v\nf{T_{I}} \in ideal(P_T)$.
      \item $u_{k}  \red{}{\lr}{}{T_{I}} v$ with $(a\imath(a),
        \lambda) \in T_{I}$.
\\
             Without loss of generality we can assume
              $u_k=xa\imath(a)y$ for some $x,y \in \Sigma^*$ and $v=xy$, i.e.
              $u_k\nf{T_{I}}=v\nf{T_{I}}$ and therefore
              $u\nf{T_{I}}-v\nf{T_{I}} \in ideal(P_T)$.
      \end{enumerate}
$2 \R 1:$ \\
 We have to show that $u\nf{T_{I}}-v\nf{T_{I}} \in ideal(P_T)$
  implies $u \red{*}{\lr}{}{T \cup T_{I}} v$.\\
 We know $u\nf{T_{I}}-v\nf{T_{I}}= \sum_{j=1}^{n} d_j \skm x_j \mrm
  (l_{i_j} - r_{i_j}) \mrm y_j$, where
  $d_j \in \myk, x_j,y_j \in \free_{fg}$.
 Therefore, by  showing the following stronger result we are done:
 A representation
 $ u - v = \sum_{j=1}^m p_j$ where $p_j = c_j \skm (w_j -w'_j)$,
 $c_j \in \myk$, $u,v,w_j,w'_j \in \free_{fg}$ and
 $w_j \red{+}{\lr}{}{T} w'_j$ implies 
 $u \red{*}{\lr}{}{T} v$.
 The proof is similar to the proof of theorem \ref{theo.wp}.
\\
\qed
%
Hence, the congruence problem for two-sided ideals in group rings is 
 also undecidable.

Furthermore, attention must be given to the set of relations
 defining our monoid, i.e., 
 in the following we will assume that
 $(\Sigma , T)$ is a finite, convergent, and even reduced presentation
 of a monoid $\m$.
As before, $\free$ denotes the free monoid generated by $\Sigma$ with 
 concatenation as multiplication.
Let $P_T = \{ l - r \mid (l,r) \in T \}$ be the set of polynomials 
 in $\myk[\m]$ related to $T$.
Further let ${\tilde T} = \{ (xl,xr) \mid (l,r) \in T, x \in \free
 \mbox{ and no proper 
 prefix of $xl$ is $T$-reducible}\}$ denote the prefix--rewriting
 system belonging to $T$ as
 described in \cite{KuMa89} and 
 $P_{{\tilde T}} = \{ xl-xr \mid (xl,xr) \in {\tilde T} \}$.

Then again the monoid ring $\myk[\m]$ can be expressed as a quotient,
 namely of the free monoid ring $\myk[\free]$.
%
\begin{lemma}~\\
{\sl
\begin{enumerate}
\item $P_{{\tilde T}}$ is confluent regarded as a set of polynomials
  in $\myk[\free]$.
\item $ideal^{\myk[\free]}(P_{{\tilde T}}) = ideal_r^{\myk[\free]}(P_{{\tilde T}})$ in $\myk[\free]$.
\item The quotient $\myk[\free]/ideal_r^{\myk[\free]}(P_{{\tilde T}})$ is a ring.  
\item The monoid ring $\myk[\m]$ is isomorphic to the quotient ring 
        $\myk[\free]/ideal_r^{\myk[\free]}(P_{{\tilde T}})$.
\end{enumerate}
}
\end{lemma}
\Ba{}~\\
\begin{enumerate}
\item Since the prefix reduction induced by  $P_{{\tilde T}}$ is
       Noetherian, in order to show
       confluence, we only have to take a look at critical pairs 
       of different polynomials
       $xl_i-xr_i,x'l_j-x'r_j \in P_{{\tilde T}}$, caused by a
       superpostion $xl_i=x'l_jz$, where $z \in\Sigma^*$.
\\
      We can distinguish two cases:
      \begin{enumerate}
      \item Let $|x|<|x'|$, i.e., $x'=xw, w \in\Sigma^* - \{ \lambda \}$.
\\
            Looking at $xl_i=xwl_jz$ we get $l_i=wl_jz$ contradicting
             that  $T$ is reduced.
      \item Let  $|x|\geq |x'|$, i.e., $x=x'w, w \in\Sigma^*$.
\\
            Looking at $x'wl_i=x'l_jz$ we have to consider two cases.
\\
            In case $z \neq \lambda$ we find that $x'l_j$ is a proper
             prefix of $xl_i$ and as $x'l_j$
             is $T$--reducible, this is a contradiction to the
             definition
             of  $P_{{\tilde T}}$.\\
            The case $z= \lambda$, $w \neq \lambda$ likewise gives 
             us a contradiction to $T$ being reduced, as $wl_i=l_j$.
\\
            In case $z= \lambda$, $w = \lambda$ likewise we get
             a contradiction to $T$ being reduced, by $l_i=l_j$.
      \end{enumerate}
      Hence the set  $P_{{\tilde T}}$ leads to no superpositions, and therefore is confluent.
\item $ideal_r^{\myk[\free]}(P_{{\tilde T}}) \subseteq
       ideal^{\myk[\free]}(P_{{\tilde T}})$ follows at once.
\\
       To show $ideal^{\myk[\free]}(P_{{\tilde T}}) \subseteq 
        ideal_r^{\myk[\free]}(P_{{\tilde T}})$ it suffices to prove that
        $x \in \free$ and $yl-yr \in P_{{\tilde T}}$ implies
        $xyl-xyr \in  ideal_r(P_{{\tilde T}})$.
\\
       In case $xyl-xyr \in P_{{\tilde T}}$ there is nothing to show.
\\
       Suppose  $xyl-xyr \not\in P_{{\tilde T}}$.
       \begin{enumerate}
       \item Assuming $xyl=x_1l'y_2l$, where $x_1l'$ is the first
              proper $T$--reducible prefix of  $xyl$,
              we get the following reduction sequences, where
              $\Longrightarrow$ stands for leftmost reduction:
              $$x_1r'y_2r \Longleftarrow_T \underline{x_1l'}y_2r=
              xyr \longleftarrow_T
              xy\underline{l}=\underline{x_1l'}y_2l
              \Longrightarrow_T x_1r'y_2l$$
              and as $T$ is complete there is a $z \in IRR(T)$ such that
              $x_1r'y_2r \red{*}{\Longrightarrow}{}{T} z 
              \red{*}{\Longleftarrow}{}{T}  x_1r'y_2l$.
             It is important that  we find $z$ by every reduction strategy,
              especially by leftmost reduction.
             This means we can find the normal form $z$ of  $xyl$
              respectively $xyr$ by using leftmost reduction only.
\\
             Since  leftmost reduction in $T$ means
              $ul_1v \Rightarrow_T ur_1v, (l_1,r_1) \in T,
              u,v \in \Sigma^*$ and no proper
              prefix of $ul_1$ is $T$--reducible,
              this can be compared to subtracting $ul_1v-ur_1v$ from
              $ul_1v$ in  $\z[{\cal F}(\Sigma)]$, where
              $ul_1-ur_1 \in  P_{{\tilde T}}$.
             Therefore $ul_1v =ur_1v +h$ for some
              $h \in  ideal_r^{\myk[\free]}(P_{{\tilde T}})$.
             Hence $xyl = z +g, xyr = z +g'$, for some
              $g,g' \in  ideal_r^{\myk[\free]}(P_{{\tilde T}})$ giving us 
              $xyl -xyr \in  ideal_r^{\myk[\free]}(P_{{\tilde T}})$. 
       \item Assuming $xyl=x_1l'l_2$, where $x_1l'$ is the first proper 
              $T$--reducible prefix of  $xyl$,
              we get the following reduction sequences
              (again $\Longrightarrow$ stands for leftmost reduction):
              $$xyr \leftarrow_T xy\underline{l}=
              \underline{x_1l'}l_2 \Longrightarrow_T x_1r'l_2$$
              and as $T$ is complete there is a $z \in IRR(T)$ such that
              $xyr \red{*}{\Longrightarrow}{}{T} z 
              \red{*}{\Longleftarrow}{}{T}  x_1r'l_2$.
             As above we can conclude  
              $xyl -xyr \in  ideal_r^{\myk[\free]}(P_{{\tilde T}})$.
       \end{enumerate}
\item This follows immediately as
       $ideal^{\myk[\free]}(P_{{\tilde T}}) =
        ideal_r^{\myk[\free]}(P_{{\tilde T}})$ in $\myk[\free]$ and
       $\myk[\free]$ is a ring.
\item Looking at the equivalences induced on $\Sigma^*$ by 
       $\red{*}{\lr}{}{T}$, $\red{*}{\lr}{}{P_T}$
       and $\red{*}{\lr}{}{P_{{\tilde T}}}$, the confluence of $T$ gives us 
        $\red{*}{\lr}{}{T}=\red{*}{\lr}{}{P_T}=
        \red{*}{\lr}{}{P_{\tilde T}}$ on $\Sigma^*$.
      Now let us look at the natural homomorphisms
       $\varphi_T : \free \myr \myk[\m]$ and 
       $\varphi_{P_{{\tilde T}}} : \free \r
       \myk[\free]/ideal_r(P_{{\tilde T}})$
       defined by
      $$\varphi_T(x) = \left\{ \begin{array}{r@{\quad:\quad}l}
                  \lambda & x=\lambda \\
                  w \downarrow_T & x=w \in \Sigma^+ \\
                  \sum_{i=1}^k c_i \skm \varphi_T(w_i) & 
                               x=\sum_{i=1}^k c_i \skm w_i,
                  \end{array} \right .  $$
      $$ \varphi_{P_{{\tilde T}}}(x) = \left\{ \begin{array}{r@{\quad:\quad}l}
                  \lambda & x=\lambda \\
                  w \downarrow_{P_{{\tilde T}}} & x=w \in \Sigma^+ \\
                  \sum_{i=1}^k c_i \skm \varphi_{P_{{\tilde T}}}(w_i)
                  &
                  x=\sum_{i=1}^k c_i \skm w_i,
                  \end{array} \right .  $$
       for $c_i \in\myk, w_i \in\Sigma^*$.
      Both homomorphisms are surjective and
      $\mbox{ Image}(\varphi_T) \cong \mbox{ Image}(\varphi_{P_{{\tilde T}}})$.
      Hence $\myk[\m] \cong \myk[\free]/ideal_r^{\myk[\free]}(P_{{\tilde T}})$.
\end{enumerate}
\qed
%
Thus we have set up a one-to-one correspondence between monoid rings
 and quotient structures of free monoid rings.
Rephrasing the definitions for multiplication, addition and reduction
 in the quotient structure of the previous section we get the
 following operations, where, as before, we assume that 
 $p \in \myk[X_1, \ldots, X_n]/ideal(P_{T})$ is in normal form with
 respect to $P_T$.
%
\begin{definition}~\\
{\rm 
Let $p,q \in \myk[\free]/ideal^{\myk[\free]}(P_{T})$.
Then we can define addition and multiplication as follows:
\begin{enumerate}
\item $p +' q := (p + q)\nf{P_T}$
\item $p \mrm ' q := (p \mrm q)\nf{P_T}$
\end{enumerate}
where $+$ and $\mrm$ are the corresponding ring operations in
 $\myk[\free]$.
}
\end{definition}
%
Then $\myk[\free]/ideal^{\myk[\free]}(P_{T})$ together with $+'$ and 
 $\mrm '$ is a ring with unit.
We will now introduce reduction to this structure.
%
\begin{definition}~\\
{\rm
Let $p,q,g \in \myk[\free]/ideal^{\myk[\free]}(P_{T})$ and
 $\red{}{\myr}{}{}$ Mora's reduction as defined in
 \ref{def.red.mora}.
Then we set
$p \red{}{\myr}{}{g} q$ if there exists a polynomial
 $q' \in \myk[X_1, \ldots, X_n]$ such that
 $p \red{}{\myr}{}{g} q'$ and $q = q'\nf{P_T}$.
\\
We can define $\red{*}{\myr}{}{}, \red{+}{\myr}{}{}$, and
 $\red{n}{\myr}{}{}$ as usual.
Reduction by a set $F \subseteq \myk[\free]/ideal^{\myk[\free]}(P_{T})$ 
 is denoted by
 $p \red{}{\myr}{}{F} q$ and stands for 
 $p \red{}{\myr}{}{g} q$ for some $g \in F$,
 also written as  $p \red{}{\myr}{}{g \in F} q$.
}
\end{definition}
%
Then for this reduction we can state:
\begin{lemma}~\\
{\sl
Let $F \subseteq \myk[\free]/ideal^{\myk[\free]}(P_{T})$ and
 $p,q \in \myk[\free]/ideal^{\myk[\free]}(P_{T})$.
\begin{enumerate}
\item $\red{}{\myr}{}{F} \subseteq \red{*}{\myr}{}{F \cup P_T}$.
\item $p \red{}{\myr}{}{F} q$ implies $p > q$.
\item $\red{}{\myr}{}{F}$ is Noetherian.
\end{enumerate}
}
\end{lemma}
%
But although $\myk[\free]/ideal^{\myk[\free]}(P_{T})$ still is a Noetherian ring,
 many other properties of reduction are lost.
%
\begin{lemma}~\\
{\sl
Let $p,q,h \in \myk[\free]/ideal^{\myk[\free]}(P_{T})$, $h \neq 0$.
\begin{enumerate}
\item $p < q$ no longer implies $p \mrm ' h < q \mrm ' h$.
\item $p \red{}{\myr}{}{q}$ no longer implies $p \mrm ' h
  \red{}{\myr}{}{q}$.
\item $p \red{}{\myr}{}{p} 0$ no longer implies $p \mrm ' h
  \red{}{\myr}{}{p} 0$.
\item $\{ p \}$ need not be a Gr\"obner basis.
\end{enumerate}
}
\end{lemma}
%
We now can give a definition for Gr\"obner bases.
%
\begin{definition}~\\
{\rm
A set $G \subseteq \myk[\free]/ideal(P_T)$ is said to be a {\em
 Gr\"obner basis}\/ of an ideal generated by a set 
 $F  \subseteq \myk[\free]/ideal(P_T)$, if
\begin{enumerate}
\item $ideal(G) = ideal(F)$
\item $\red{*}{\myr}{}{G}$ is confluent.
\end{enumerate}
}
\end{definition}
%
The following lemma describes a way to compute such bases.
%
\begin{lemma}~\\
{\sl
Let $P_T$ be a Gr\"obner basis\footnote{Note that in case $T$ is
 confluent, then $P_T$ is a Gr\"obner basis.},
 $F \subseteq \myk[\free]/ideal^{\myk[\free]}(P_{T})$
 and let $\red{}{\myr}{}{F \cup P_T}$ be confluent on $\myk[free]$.
Then $\red{}{\myr}{}{F}$ is also confluent.
}
\end{lemma}
%
The converse is not true.
But we can compute a Gr\"obner basis as follows:

Compute a Gr\"obner basis $G'$ of $F \cup P_T$ in
 $\myk[\free]$ with respect to Mora's
 reduction without changing the polynomials in $P_T$.
Then the set $G := G' \backslash P_T$ is a Gr\"obner basis
 of $F$ in $\myk[\free]/ideal^{\myk[free]}(P_T)$.
Computing a Gr\"obner basis of $F \cup P_T$ three kinds of
 s-polynomials can arise:
\begin{enumerate}
\item $f,g \in P_T$:
\\
      Then the corresponding s-polynomial can be omitted in case
       $P_T$ is already a Gr\"obner basis.
\item $f,g \in F$:
\\
      Then the s-polynomial corresponds to the prefix
       s-polynomial as defined in section \ref{section.} in case
       we restrict ourselves to prefix right reduction instead of
       Mora's reduction.
\item $f \in F$, $g \in P_T$:
\\
      Then the s-polynomial corresponds to the process of
       saturating $f$, in particular to the step of overlapping
       the head term of $f$ with the rule $(l,r) \in P_{\tilde{T}}$
       where $g = l-r$.
\end{enumerate}
We end up with a characterization of Gr\"obner bases as follows:
%
\begin{theorem}~\\
{\sl 
Let $G \subseteq \myk[\free]/ideal^{\myk[\free]}(P_T)$.
$G$ is a Gr\"obner basis if
\begin{enumerate}
\item for all $f,g \in G$, $spol(f,g) \red{*}{\myr}{}{G} 0$ and
\item for all $f \in G$, $g \in P_T$, $spol(f,g) \red{*}{\myr}{}{G} 0$.
\end{enumerate}
}
\end{theorem}
%
In fact the two reductions $\red{}{\myr}{}{}$ and $\red{}{\myr}{p}{}$ are
closely related and one can show the equivalence of the above
characterization to the following
%
\begin{theorem}~\\
{\sl 
Let $G \subseteq \myk[\m]$.
$G$ is a Gr\"obner basis if
\begin{enumerate}
\item for all $f,g \in G$, $spol_p(f,g) \red{*}{\myr}{p}{G} 0$ and
\item for all $f \in G$, every right multiple of $f$ has a
      prefix standard representation with respect to $G$.
\end{enumerate}
}
\end{theorem}
%
\begin{example}~\\
{\rm
Let the monoid $\m$ be presented by
 $\Sigma = \{ a,b,c \}$ with $c \succ b \succ a$ and
 $T = \{ ba \myr ab, ca \myr ac, cb \myr bc \}$.
We will investigate the set $F= \{ abc + \lambda \}$.
\\
In $\myk[\m]$ the set $F$ itself is a Gr\"obner basis for
 the ideal generated by $F$.
In $\myk[\free]/ideal_r(P_T)$ no finite Gr\"obner basis exists,
 but the set $G = \{ ab^ic + b^i | i \in \n \}$ is an infinite
 one.
}
\end{example}
%

!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
TODO:

Vergleich der Reduktionen und Gr\"obner Basen

!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

Note that the isomorphism need not be reduction preserving
 as in general reduction in the
 quotient ring can also be done in $\myk[\m]$ but not vice versa.
But a Gr\"obner basis in the quotient ring
 is also a Gr\"obner basis in $\myk[\m]$.
%
\begin{example}~\\
{\rm
Let $\Sigma = \{x_1,x_2,x_3 \}, T = \{ x_ix_j \myr x_jx_i \mid 1 \leq j<i \leq 3 \}$.
Reduction in $\z[\h]$ can be defined as in definition \ref{def.redr}.
(Prefix) reduction in $\z[{\cal F}(\Sigma)]/ideal_r(P_{{\tilde T}})$
is defined as  $p_1 \red{}{\leadsto}{}{p_2} p_3$ if
 $HC(p_1)= a \cd HC(p_2) + b, a,b \in \z$,$b$ a remainder of $HC(p_2)$,$HT(p_1)=HT(p_2)x$
 for some $x\in \h$ and $p_3$ is the normal form of $p_1-a \cd p_2 \cd x$ modulo $ideal_r(P_{{\tilde T}})$.
\\
Now looking at $p = x_1^2x_2 + x_3, q = x_1^3x_2 + x_1$ we get
 $q \red{}{\myr}{}{p}  x_1^3x_2 + x_1 - ( x_1^2x_2 + x_3) \cd x_1 = -x_1x_3 + x_1 $ in $\z[\h]$
 but $q \nred{}{\leadsto}{}{p}$ in  $\z[{\cal F}(\Sigma)]/ideal_r(P_{{\tilde T}})$.
}
\end{example}
%
Now we state some useful facts which give some more insight into our problems:
\begin{enumerate}
\item $\myk[X_1, \ldots , X_n]$ allows the computation of Gr\"obner bases of
 ideals via reduction as given in \cite{Bu85}.
\item $\myk[\free]$  allows the computation of Gr\"obner bases of right
  ideals via right reduction but not of ideals in general
 (see the previous section or \cite{Mo85}).
\item $\myk[X_1, \ldots , X_n]/ideal_r(P_{T})$ allows the computation of finite
       Gr\"obner bases of ideals via right reduction
       (see the previous section or (Dei{\ss})).
\item $\myk[\free]/ideal_r(P_{T})$ in general does not allow the computation of
       finite Gr\"obner bases of right ideals via right reduction
 ( for example if $T$ includes one commutative  rule).
\end{enumerate}
%

Since 1965 the existence of finite Gr\"obner bases has been shown for several structures.
Authors as Mora, Baader, Kandri-Rody, Weispfenning, Madlener, Reinert, and Rosenmann have investigated the
 situation for special non-commutative polynomial rings.
They have shown that in many cases finitely generated one or two-sided
ideals admit finite Gr\"obner bases, e.g.\  for free monoid rings,
solvable polynomial rings, skew polynomial rings, free group rings and
plain group rings (compare the introduction of this paper).
\\
However, the question whether a finite Gr\"obner basis with respect to reduction, as e.g.\  
 specified by Mora in \cite{Mo85}, exists for a finitely generated ideal in the
 free monoid ring, is undecidable.
%
\begin{theorem}~\\
{\sl
It is undecidable, whether a finitely generated ideal has a finite Gr\"obner basis in
 the free monoid ring $\myk[\{ s,t \}^*]$ with respect to reduction as defined in 
 definition \ref{def.red.mora}.
}
\end{theorem}
\Ba{}
Using the technique described by \'{O}'D\'{u}nlaing in \cite{OD83} Otto has shown that the following
 question is undecidable (\cite{Ot93}):
\\
\\
{\sl
Let $\succ$ be a compatible well-founded partial ordering on $\{s,t \}^*$ such that
 $s \succ \lambda$ and $t  \succ \lambda$ both hold. 
\\
Given a finite Thue system $T$ on $\{ s,t \}$.
Is there a finite and confluent system $T'$ on $\{ s,t \}$ that is equivalent to
                 $T$ and that is based on $\succ$?
}
\\
\\
We can show that the answer for $T$ is ``yes'' if and only if $P_{T} = \{ l - r | (l,r) \in T, l \succ r \}$
 has a finite Gr\"obner basis in   $\myk[\{ s,t \}^*]$ with respect to $\succ$.
\\
If there is an equivalent, finite presentation $(\{s,t\} , T')$  convergent with respect to
 $\succ$, then the set $P_{T'}= \{ l-r \mid (l,r) \in T' \}$ is a finite Gr\"obner basis of $P_{T}$ in 
 $\myk[\{ s,t \}^*]$.
This follows as the Thue reduction $\red{}{\lr}{}{T'}$ can be
simulated by the symmetric closure of the reduction
$\red{}{\lr}{}{P_T}$ in $\myk[\{ s,t \}^*]$
 (compare definition \ref{def.red.mora}).
\\
It remains 
 to show that in case $P_{T}$ has a finite Gr\"obner basis in $\myk[\{ s,t \}^*]$ there exists
 a finite Gr\"obner basis $G$ such that for all $g \in G$ we have $g = u-v$, where $u,v \in \{s,t\}^*$, and
 $u \red{*}{\lr}{}{T} v$.
Then $(\{s,t\} , T)$ has  an equivalent, convergent, finite presentation $(\{s,t\} , T')$, namely
 $T' = \{ (u,v) \mid u-v \in G \}$, since the reduction $\red{}{\myr}{}{}$
 in $\myk[\{ s,t \}^*]$ as defined above
 can be compared to a transformation step in a Thue system when restricted to polynomials of the form
 $u-v$.
\\
First we show that in case a finite set $F$ has a finite Gr\"obner basis in  $\myk[\{ s,t \}^*]$ the
 following procedure also computes a finite Gr\"obner basis of $F$ (compare \cite{Mo85}).

\procedure{Completion in $\myk[\{ s,t \}^*]$}%
{\begin{tabbing}
XXXXX\=XXXX \kill
\removelastskip
{\bf Given:} \> $F \subseteq  \myk[\{ s,t \}^*]$ finite \\
{\bf Find:} \> $\gb(F)$, a Gr\"obner basis of $F$.
\end{tabbing}
\begin{tabbing}
XXXXXX\= XXXXX\= XXXXX \= XXXXX \=\kill
$G$ := $F$; \\
$B$ := $\{ (q_{1}, q_{2}) \mid q_{1}, q_{2} \in G \}$; \\
{\bf while} $B \neq \emptyset$ {\bf do} \\
\>      $(q_{1}, q_{2}) := {\rm remove}(B)$; \\
\>      {\bf for all} $h \in spols(q_{1}, q_{2})$ {\bf do}  \\
\> \> {\scriptsize \% $spols(q_1,q_2)= \{(HC(q_1)^{-1} \skm x \mrm q_1 \mrm y -
               HC(q_2)^{-1} \skm q_2 \mid xHT(q_1)y=HT(q_2) \} \cup$} \\
\> \> {\scriptsize \%   $\{HC(q_1)^{-1} \skm q_1 \mrm y -
               HC(q_2)^{-1} \mrm x \mrm q_2 
             \mid HT(q_1)y=xHT(q_2) , |HT(q_1)| < |x|\}$} \\
\> \>    $h' := {\rm headnormanlform}(h, G)$; \\
\> \>   {\bf if} $h' \neq 0$  \\
\> \> \>  {\bf then}     $G := G \cup \{ h' \}$; \\
\> \> \>       $B := B \cup \{ (f, h'), (h',f) \mid f \in G \}$; \\
\>  {\bf endfor} \\
{\bf endwhile} \\
$\gb (F):= G$
\end{tabbing}}
%where  $remove$ removes an element from a set using a fair strategy,
% $hnf(h,G)$ computes a ``head normal form'' of $h$ with respect to
% $G$, and 
% $spols(q_1,q_2)= \{(HC(q_1)^{-1} \skm x \mrm q_1 \mrm y -
% HC(q_2)^{-1} \skm q_2 
% \mid xHT(q_1)y=HT(q_2) \} \cup \{HC(q_1)^{-1} \skm q_1 \mrm y -
% HC(q_2)^{-1} \mrm x \mrm q_2 
% \mid HT(q_1)y=xHT(q_2) \}$.

Now let $\tilde{G}$ be a finite Gr\"obner basis of $P_{T}$ with
 $HT(\tilde{G})=\{HT(g) \mid g \in \tilde{G} \} = \{ t_1, \ldots , t_k
 \}$. 
Let $H_{t_i} = \{ xt_iy \mid x,y \in \Sigma^* \}$, then
$HT(ideal(P_{T}))= \bigcup_{i=1}^k H_{t_i}$, since 
 all polynomials in $ideal(P_{T})$ reduce to zero by $\tilde{G}$.
Further our procedure is correct and, therefore, for each $t_i$ there
has to be at least 
 one $g_i$ added to $G$ such that $t_i=xHT(g_i)y$ for some $x,y \in
 \Sigma^*$, i.e. $HT(g_i)$ divides $t_i$. 
Note that as soon as all such $g_i$ are added to $G$, we have
 $HT(ideal(G)) = \bigcup_{i=1}^k H_{t_i}=HT(ideal(P_{T}))$ and since
 for all further computed polynomials  $h'$
 we know  $h'$ is in normal form with respect to $G$ and $h' \in
 ideal(P_{T})$ implying $h'=0$.
\\
It remains to show that in case $P_{T}$ has a finite Gr\"obner basis,
the finite output $\gb(P_{T})$ of our 
 procedure has the desired structure such that for all $g \in
 \gb(P_{T})$, $g=u-v$ where $u,v \in \Sigma^*$, and 
 $u \red{*}{\lr}{}{T} v$.
\\
Since all polynomials in $P_T$ have the desired property let us look
at the polynomials added to $G$: 
Let us assume all polynomials in $G$ have the desired structure and a
new polynomial $g$ is added. 
In case $g$ is due to s--polynomial computation of two polynomials
$u_1-v_1$,$u_2-v_2$ we do not 
 lose our structure.
The same is true for computing the  head normal form of a polynomial
$u-v$ via 
 a set of polynomials having the same structure.
Further $u \red{*}{\lr}{}{T} v$ is inherited within these operations
(compare also the proof of theorem 
 \ref{theo.wp}).
\\
\qed
%
In restricting our attention to right ideals, we find that the
generalized word problem can be 
 reduced to the congruence problem for right ideals in a group ring.
%Therefore, in this surrounding finite Gr\"obner bases allow the
% solvability of the  subgroup problem.
\begin{definition}~\\
{\rm
Let $\g$ be a group, $S \subseteq \g$ and $\left< S \right>$ denote
 the subgroup generated by $S$. 
The {\em generalized word problem}\/ or {\em subgroup problem}\/ is to
 determine, given $w \in \g$, whether $w \in \left< S \right>$. 
} 
\end{definition}
%
Let $(\Sigma , T)$ be a group system presenting a group $\g$.
Further let $S = \{ u_1, \ldots , u_n \}$ be a subset of $\g$ and $P_S
 = \{ u_i - 1 \mid u_i \in S \}$. 
%
\begin{theorem}~\\
{\sl
Let $S \subseteq \g$ and $\myk[\g]$ the corresponding group ring. 
Then the following statements are equivalent:
\begin{enumerate}
\item $w \in  \left< S \right>$ 
\item $w-1 \in ideal_r(P_S)$
%\item $w-1 \red{*}{\myr}{r}{\gb(P_S)} 0 \subseteq \myk[\g]$  
\end{enumerate}
}
\end{theorem}
\Ba{}~\\
$1 \R 2:$ \\
      Let $w = u_{i_1}\mm \ldots\mm u_{i_k}$.
\\      
      We show $w-1 \in ideal_r(P_S)$ by induction on $k$.
\\
      In the base case $k=0$ there is nothing to show, as $w=1 \in  \left< S \right>$\footnote{Note that $1 = 1 \skm \lambda = \lambda$} and $0 \in ideal_r(P_S)$.
\\
      Suppose  $w = u_{i_1}\mm \ldots\mm u_{i_{k+1}}$ and $
      u_{i_1}\mrm \ldots\mrm u_{i_k}-1 \in ideal_r(P_S)$.
\\
      Then $( u_{i_1}\mrm \ldots\mrm u_{i_k}-1) \mrm u_{i_{k+1}} \in ideal_r(P_S)$ and, since 
      $ u_{i_{k+1}}-1 \in ideal_r(P_S)$, we get
      $( u_{i_1}\mrm \ldots\mrm u_{i_k}-1) \mrm u_{i_{k+1}} +
      (u_{i_{k+1}} - 1) = w-1 \in ideal_r(P_S)$.
\\
\\
$2 \R 1:$ \\
       We have to show that $w-1 \in ideal_r(P_T)$ implies $w \in  \left< S \right>$.\\
       We know $w-1 = \sum_{j=1}^{n} d_j \skm (u_{i_j} -1) \mrm x_j$, where
       $d_j \in \myk, x_j \in \g$.
       Therefore, by  showing the following stronger result we are done:
       A representation
       $ w - 1 = \sum_{j=1}^m p_j$ where $p_j = c_j \skm (w_j -w'_j)$,
       $c_j \in \myk$,$w_j \neq w'_j$ and $w_j \mm  (w'_j)^{-1} \in \left< S \right>$ implies 
       $w \in \left< S \right>$.
       \\
       Let $w - 1 = \sum_{j=1}^m p_j$ be such a representation.
       Further let $\succ$ be  an arbitrary total well-founded ordering
       on $\g$.
       \\
       Depending on the  representation $\sum_{j=1}^m p_j$  and the ordering $\succ$ we define
       $t = max \{w_j,w'_j   \mid j = 1, \ldots m  \}$  and
       $K =$ number of $p_j$ containing $t$ as a term.
       \\
       We will show our claim by induction on $(m,K)$, where 
       $(m',K') < (m,K)$ if and only if $m'<m$ or $(m'=m$ and $K'<K)$.
\\
       In case $m=0$, $w-1=0$ implies $w=1$ and hence $w \in  \left< S \right>$.
       \\
       Now let $m>0$.
\\
       In case $K=1$, let $p_k$ be the polynomial containing $t$\footnote{We either have $p_k=c_k \skm (t-w'_k)$ or $p_k=c_k \skm (w_k - t)$, where $c_k \in \{ 1, -1 \}$.}.
       Without loss of generality we can assume $p_k=t-w'_k$.
       Using $p_k$ we can decrease $m$ by subtracting $p_k$ from $w-1$ giving us
       $w'_k-1 = \sum_{j=1,j \neq k}^{m} p_j$.
       Since $t \mm   (w'_k)^{-1} \in \left< S \right>$ and our induction hypothesis yields
       $w'_k \in \left< S \right>$,
       we get $w=t=t \mm  (w'_k)^{-1} \mm  w'_k \in \left< S \right>$.
       \\
       In case $K>1$ there are two polynomials $p_k,p_l$ in the corresponding representation
        and without loss
        of generality we can assume $p_k = c_k \skm( t - w'_k)$ and $p_l = c_l \skm (t -w'_l)$.
       \\
       If $w'_k = w'_l$  we can immediately decrease $m$ 
        by substituting the occurrence of $p_k+p_l$  by $(c_k + c_l) \skm p_l$.
\\
       Otherwise we can proceed as follows:
       \begin{eqnarray*}
         p_k + p_l & = & p_k \underbrace{-  c_k \skm c_l^{-1} \skm p_l + c_k  \skm c_l^{-1} \skm p_l}_{=0} + p_l \\
                   & = & \underbrace{(-c'_k \skm w'_k + c_k  \skm w'_l)}_{p'k} + (c_k \skm c_l^{-1} +1) \skm p_l \\
       \end{eqnarray*}
       where $p'_k = c_k \skm (w'_l - w'_k)$, $w'_k \neq w'_l$
       and $w'_k \mm  (w'_l)^{-1} \in\left< S \right>$, since
       $w'_k \mm  t^{-1},t \mm  (w'_l)^{-1} \in\left< S \right>$ and 
       $w'_k \mm  (w'_l)^{-1}=w'_k \mm  t^{-1} \mm  t \mm  (w'_l)^{-1}$.
      In case $c_k \skm c_l^{-1} + 1=0$, i.e., $c_k=-c_l$, $m$ is decreased.
      On the other hand $p'_k$ does not contain $t$, i.e. if $m$ is
      not decreased $K$ is.
\\
\qed
%
%However, the previous theorems show that in case a finite Gr\"obner basis can be computed for
% these finitely generated ideals, it
% can be used to solve the word problem respectively the generalized word problem.
%In the following section we will investigate some structures which allow finite Gr\"obner bases
% for finitely generated right ideals.

%
\section{Odd Bits on Gr\"obner Bases}
%
Further structural information on Gr\"obner bases:
\\
For $F \subseteq \z[\h]$ let $HT(ideal_r(F))$ denote the set of the head terms of all polynomials in  $ideal_r(F)$.
In the polynomial ring $R[x_1, \ldots,x_n]$ we know that $HT(ideal(F))$ itself is an ideal,
 in fact the ideal generated by $HT(G)$, where $G$ is a Gr\"obner basis of $ideal(F)$.
This is cruical when proving termination of Buchbergers algorithm.
Unfortunately this is no longer true for arbitrary monoid rings.
%
\begin{example}~\\
{\rm
Let $\Sigma = \{ a,b \}$, $T = \{ a^2 \myr \lambda, b^2 \myr \lambda , ba \myr ab \}$ and $p=ab+ \lambda$.
Then $\{ p \}$ is a Gr\"obner basis of $ideal(p)$ but $HT(ideal(p))= \{ a, ab \} \neq HT(ideal(ab)) = \{ \lambda, a, b, ab \}$.
}
\end{example}
\begin{lemma}~\\
{\sl
There is a monoid $\h$ with a length-reducing presentation and a set $F \subseteq \z[\h]$
 such that $HT(ideal_r(F))$ is regular but
 $ideal_r(F)$ has no finite Gr\"obner basis via $\red{}{\myr}{r}{}$.
}
\end{lemma}
\Ba{}
Let $\h$ be the monoid presented by $\Sigma = \{ a,b,c,d,e,f \}$ with $a \succ b  \succ c   \succ
    d  \succ e \succ f$,
 $T = \{ abc \myr ba, fbc \myr bf, bad \myr e \}$ and $F= \{ a+f, bf+1 \}$.
\\
Then $a+f$ gives us the polynomials $\{ b^iaw_1+ b^ifw_1, b^{i+1}fdw_2+b^iew_2 \mid i \in \n,
 w_1 \in IRR(T)-bc \cd \Sigma^*, w_2 \in IRR(T) \}$ and 
 $bf+1$ gives us the polynomials $\{ b^{i+1}fw+b^iw \mid i \in \n,w \in IRR(T)-bc \cd \Sigma^* \}$.
Further we have  critical situations
 in $b^{i+1}fdw$ leading to the polynomials
 $\{ b^iew-b^ifw \red{*}{\myr}{}{} b^iew + (-1)^{i+1}fw \mid i \in\n, w \in IRR(T) \}$.
We get $HT(ideal_r(F))= \{ b^i aw_1, b^i fw_1, b^{i+1}fdw_2, b^iew_2 \mid
 i \in\n, w_1 \in IRR(T)-bc \cd \Sigma^*, w_2 \in IRR(T) \}$.
\\
$HT(ideal_r(F))$ is regular since
 $HT(ideal_r(F))=b^*aR_1 \cup b^*fR_1 \cup b^*bfdR_2 \cup b^*eR_2$, where
 $R_1= IRR(T) \cap (\bigcup_{x,y \in \Sigma \cup \{ \lambda \}, xy \neq bc} xy \cd \Sigma^*)$ and $R_2=IRR(T)$.
\\
It remains to show there is no finite Gr\"obner basis.
\\
For a Gr\"obner basis $B$ we have
 $HT(B) \subseteq HT(ideal_r(F))= \{ b^i aw_1, b^i fw_1, b^{i+1}fdw_2, b^iew_2 \mid
 i \in\n, w_1 \in IRR(T)-bc \cd \Sigma^*, w_2 \in IRR(T) \}$.
\\
Now in case $B$ is finite we can choose $N \in \n$ such that $b^Ne+(-1)^{N+1}f \not\in B$.
Then $b^Ne+(-1)^{N+1}f$ must be irreducible since for all $t,x \in IRR(T)$ we have $t \cd x = b^Ne$ iff
 $tx=b^Ne$ and no prefix of $b^Ne$ is in $HT(B)$.
\\
\qed
%
\begin{lemma}~\\
{\sl
There is a monoid $\h$ and a set $F \subseteq \z[\h]$ such that $HT(ideal_r(F))$ is not regular but
 $ideal_r(F)$ has a finite Gr\"obner basis via $\red{}{\myr}{r}{}$.
}
\end{lemma}
\Ba{}
Let $\h$ be the monoid presented by $\Sigma = \{ a,b,c,d,e \}$ with $a \succ b \succ c \succ d \succ e$,
 $T = \{ abdc \myr cba, ebdc \myr cbe, bc \myr cb \}$ and $F= \{ a+e \}$.
\\
Then $a+e$ gives us the polynomials $\{  c^ib^{i}aw+c^ib^iew \mid i \in \n, w \in IRR(T) - bdc \cd \Sigma^* \}$.
Since there are no critical situations we get $HT(ideal_r(F))= \{ c^ib^i aw \mid i \in\n, w \in IRR(T)-bdc \cd \Sigma^* \}$ which  is not regular since 
 $HT(ideal_r(F)) \cap c^*b^*a = \{ c^ib^ia \mid i \in\n \}$.
But $F$ is a Gr\"obner basis via $\red{}{\myr}{r}{}$.
\\
This is also an example for a polynomial $p$ where $HT(p) \cd IRR(T)$
is not regular, but $p$ can be saturated.
\\
\qed
%
\begin{remark}~\\
{\rm
In case $T$ is context-free-monadic for all $t \in IRR(T)$ the set $t \cd IRR(T)$ is regular.
This follows as $t \cd IRR(T) = \Delta^*(\{tx \ x \in IRR(T)\}) \cap IRR(T)$ is the intersection of regular sets.
}
\end{remark}

==> pdf.tex <==
%&latex
\input body

